BINAS: Bilinear Interpretable Neural Architecture Search

Practical use of neural networks often involves requirements on latency, energy and memory among others. A popular approach to find networks under such requirements is through constrained Neural Architecture Search (NAS). However, previous methods use complicated predictors for the accuracy of the network. Those predictors are hard to interpret and sensitive to many hyperparameters to be tuned, hence, the resulting accuracy of the generated models is often harmed. In this work we resolve this by introducing Bilinear Interpretable Neural Architecture Search (BINAS), that is based on an accurate and simple bilinear formulation of both an accuracy estimator and the expected resource requirement, together with a scalable search method with theoretical guarantees. The simplicity of our proposed estimator together with the intuitive way it is constructed bring interpretability through many insights about the contribution of different design choices. For example, we find that in the examined search space, adding depth and width is more effective at deeper stages of the network and at the beginning of each resolution stage. Our experiments show that BINAS generates comparable to or better architectures than other state-of-the-art NAS methods within a reduced marginal search cost, while strictly satisfying the resource constraints.

==> abstract_pre.tex <==
\begin{abstract}
Realistic use of neural networks often requires adhering to multiple constraints on latency, energy and memory among others.
A popular approach to find fitting networks is through constrained Neural Architecture Search (NAS), however, previous methods optimize a very complicated objective function to be a surrogate prediction model for the accuracy of the network. 
Those predictors are both expensive to obtain and hard to interpret and optimize, hence, the resulted accuracy of the generated models is harmed.
In this work we resolve this by introducing \textit{Quadratic constraints quadratic Programming NAS (QPNAS)}, that is based on an accurate and simple quadratic formulation of both the accuracy predictor and the expected resource requirement, together with a scalable search method with theoretical guarantees. Many insights about the contribution of different design choices are deduced due to the interpretability of the proposed accuracy predictor.
Our experiments show that QPNAS generates 
comparable to or 
better architectures than other state-of-the-art NAS methods within a reduced search cost, while strictly satisfying the resource constraints.
\end{abstract}

==> big_table.tex <==
\begin{table}[t]
\small
    \centering
    \begin{tabular}{c|l|c|c|c|}
    & Model & \makecell[c]{Latency \\ (ms)} & \makecell[c]{Top-1 \\ (\%)} & \makecell[c]{Total  Cost\\(GPU hours)}%Search + Training \\ Cost (GPU hours)}
    \\ \toprule
         \multirow{17}{*}{\rotatebox[origin=c]{90}{NVIDIA P100 GPU (batch:64)}}
         & MobileNetV3 & 28 & 75.2 & 180N \\ 
         & TFNAS-D & 30 & 74.2  & 236N \\ 
         & HardCoRe A & 27 & 75.7  & 400 + 15N\\
         & \textbf{Ours 25 ms} & \textbf{26} & \textbf{76.1} & 435 + \textbf{8N}\\
         & \textbf{Ours 25 ms} & \textbf{26} & \textbf{76.6} & 435 + 15N\\
         \cline{2-5}
         
         & MnasNetA1 & 37 & 75.2  & 40,000N \\
         & MnasNetB1 & 34 & 74.5  & 40,000N \\ 
         & FBNet & 41 & 75.7  & 576N \\ 
         & SPNASNet & 36 & 74.9  & 288 + 408N\\ 
         & TFNAS-B &  44 & 76.3  & 263N \\ 
         & TFNAS-C & 37 & 75.2  & 263N \\ 
         & HardCoRe B & 32 & \textbf{77.3} & 400 + 15N \\
         & \textbf{Ours 30 ms} & \textbf{31} & 76.8 & 435 + \textbf{8N} \\ 
         & \textbf{Ours 30 ms} & \textbf{31} & 77.2 & 435 + 15N \\ 
          \cline{2-5}
         
         & TFNAS-A & 54 & 76.9  & 263N \\ 
         & EfficientNetB0 & 48 & 77.3 &  \\ 
         & MobileNetV2 & 50 & 76.5  & 150N \\ 
         & HardCoRe C & 41 & \textbf{77.9}  & 400 + 15N \\
         & \textbf{Ours 40 ms} & \textbf{40} & 77.6 & 435 + \textbf{8N} \\ 
         & \textbf{Ours 40 ms} & \textbf{40} & 77.7 & 435 + 15N \\ 
         \midrule
         
         \multirow{20}{*}{\rotatebox[origin=c]{90}{Intel Xeon CPU (batch:1)}}
         
         & MnasNetB1 & 39 & 74.5 & 40,000N\\ 
         & TFNAS-B & 40 & 75.0 & 263N \\ 
         & SPNASNet & 41 & 74.9 & 288 + 408N\\ 
         & OFA CPU\footnotemark & 42 & 75.7 & 1200 + 25N \\ 
         & HardCoRe A & 40 & 75.8 & 400 + 15N\\ 
         & \textbf{Ours 40 ms} & \textbf{40} & \textbf{76.1} & 435 + \textbf{8N}\\ 
         & \textbf{Ours 40 ms} & \textbf{40} & \textbf{76.5} & 435 + 15N \\ \cline{2-5}
         
         & MobileNetV3 & 45 & 75.2 & 180N \\ 
         & FBNet & 47 & 75.7 & 576N \\ 
         & MnasNetA1 & 55 & 75.2 & 40,000N \\ 
        
         & HardCoRe B & 44 & 76.4 & 400 + 15N\\ 
         & \textbf{Ours 45 ms} & \textbf{45} & \textbf{76.5} & 435 + \textbf{8N}\\ 
         & \textbf{Ours 45 ms} & \textbf{45} & \textbf{77.0} & 435 + 15\\ \cline{2-5}
         
         & MobileNetV2 & 70 & 76.5 & 150N \\ 
         & TFNAS-A & 60 & 76.5 & 263N \\ 
         & HardCoRe C & \textbf{50} & 77.1 & 400 + 15N \\ 
         & \textbf{Ours 50 ms} & \textbf{50} & 76.8 & 435 + \textbf{8N} \\ 
         & \textbf{Ours 50 ms} & \textbf{50} & \textbf{77.6} & 435 + 15N \\ \cline{2-5}
         
         & EfficientNetB0 & 85 & 77.3 &  \\ 
         & HardCoRe D & 55 & 77.6 &  400 + 15N\\
         & \textbf{Ours 55 ms} & \textbf{55} & 77.7 &  435 + \textbf{8N}\\ 
         & \textbf{Ours 55 ms} & \textbf{55} & \textbf{77.8} &  435 + 15N\\ \cline{2-5}
         
         & FairNAS-C & 60 & 77.0 & 240N \\ 
         & HardCoRe E & 61 & \textbf{78.0} & 400 + 15N\\ 
         & \textbf{Ours 60 ms} & \textbf{59} & 77.8 & 435 + \textbf{8N}\\ 
         & \textbf{Ours 60 ms} & \textbf{59} & \textbf{78.0} & 435 + 15N \\ \hline
    \end{tabular}
    \caption{ImageNet top-1 accuracy, latency and cost comparison with other methods. The total cost stands for the search and training cost of N networks.} %Latency is reported for Intel Xeon CPU and NVIDIA P100 GPU with a batch size of 1 and 64 respectively}
    \label{tab:exp}
    \vspace{-5mm}
\end{table}\footnotetext{\label{fn:ofa}Finetuning a model obtained by 1200 GPU hours.}
% \vspace{-5mm}

==> cpu_table.tex <==
\begin{table}[t]
\small
    \centering
    \begin{tabular}{c|l|c|c|c|}
    & Model & \makecell[c]{Latency \\ (ms)} & \makecell[c]{Top-1 \\ (\%)} & \makecell[c]{Total  Cost\\(GPU hours)}%Search + Training \\ Cost (GPU hours)}
    \\ \toprule
         \multirow{14}{*}{\rotatebox[origin=c]{90}{NVIDIA P100 GPU (batch:64)}}
         & MobileNetV3 & 28 & 75.2 & 180N \\ 
         & TFNAS-D & 30 & 74.2 & 236N \\ 
         & \textbf{Ours 25 ms} & \textbf{27} & \textbf{75.7} & 400 + \textbf{15N}\\ \cline{2-5}
         
         & MnasNetA1 & 37 & 75.2 & 40,000N \\
         & MnasNetB1 & 34 & 74.5 & 40,000N \\ 
         & FBNet & 41 & 75.7 & 576N \\ 
         & SPNASNet & 36 & 74.9 & 288 + 408N\\ 
         & TFNAS-B &  44 & 76.3 & 263N \\ 
         & TFNAS-C & 37 & 75.2 & 263N \\ 
         & \textbf{Ours 30 ms} & \textbf{32} & \textbf{77.3} & 400 + \textbf{15N} \\ \cline{2-5} 
         
         & TFNAS-A & 54 & 76.9 & 263N \\ 
         & EfficientNetB0 & 48 & 77.3 &  \\ 
         & MobileNetV2 & 50 & 76.5 & 150N \\ 
         & \textbf{Ours 40 ms} & \textbf{41} & \textbf{77.9} & 400 + \textbf{15N} \\ \midrule
         
         \multirow{15}{*}{\rotatebox[origin=c]{90}{Intel Xeon CPU (batch:1)}}
         
         & MnasNetB1 & 39 & 74.5 & 40,000N\\ 
         & TFNAS-B & 40 & 75.0 & 263N \\ 
         & SPNASNet & 41 & 74.9 & 288 + 408N\\ 
         & OFA CPU\footnotemark & 42 & 75.7 & 1200 + 25N \\ 
         & \textbf{Ours 40 ms} & \textbf{40} & \textbf{75.8} & 400 + \textbf{15N}\\ \cline{2-5}
         
         & MobileNetV3 & 45 & 75.2 & 180N \\ 
         & FBNet & 47 & 75.7 & 576N \\ 
         & MnasNetA1 & 55 & 75.2 & 40,000N \\ 
         
         & \textbf{Ours 45 ms} & \textbf{44} & \textbf{76.4} & 400 + \textbf{15N}\\ \cline{2-5}
         
         & MobileNetV2 & 70 & 76.5 & 150N \\ 
         & TFNAS-A & 60 & 76.5 & 263N \\ 
         & \textbf{Ours 50 ms} & \textbf{50} & \textbf{77.1} & 400 + \textbf{15N} \\ \cline{2-5}
         & EfficientNetB0 & 85 & 77.3 &  \\ 
         & \textbf{Ours 55 ms} & \textbf{55} & \textbf{77.6} &  400 + \textbf{15N}\\ \cline{2-5}
         & FairNAS-C & 60 & 77.0 & 240N \\ 
         & \textbf{Ours 60 ms} & \textbf{61} & \textbf{78.0} & 400 + \textbf{15N}\\ \hline
    \end{tabular}
    \caption{ImageNet top-1 accuracy, latency and cost comparison with other methods. The total cost stands for the search and training cost of N networks.} %Latency is reported for Intel Xeon CPU and NVIDIA P100 GPU with a batch size of 1 and 64 respectively}
    \label{tab:exp}
\end{table}\footnotetext{\label{fn:ofa}Finetuning a model obtained by 1200 GPU hours.}

==> exp_v0.tex <==
\section{Experimental Results}\label{sec:experiments}
\subsection{Validation of the Latency Formula}\label{sec:validate_latency}
Aiming at providing a practical method to accurately fit the user's resource requirements, we validate the accuracy of our latency formula (\ref{eqn:latency_formula}) by comparing its outcome to the measured latency for several models on Intel Xeon CPU and NVIDIA P100 GPU. The measurements are shown in Figure~\ref{fig:latency}, admitting a linear relation with the ratio of $1.003$ and a coefficient of determination of $R^2=0.99$. This validates the accuracy of the proposed formula.

\subsection{Evaluating the Solution of the Inner Problem $w^*$}\label{sec:evaluate_inner}
The ultimate quality measure for a generated architecture is arguably its accuracy over a test set when trained as a stand-alone model from randomly initialized weights.
Hence, relaying on the solution $w^*$ of the inner problem of (\ref{eqn:NAS_bilevel}) for searching the space (section \ref{sec:outer_problem}) requires the one-shot model equipped with $w*$ to admit correlated rankings of the accuracy of sub-netwroks extracted from it and their corresponding stand-alone accuracy.
For the evaluation of this correlation, we calculate the Kendall-Tau \cite{KendallTau} and Spearman's \cite{spearman1961general} rank correlation coefficients, denoted as $\tau$ and $\rho$ respectively.
To this end extract 18 sub-networks over the entire search space $d\in \{2,3,4\}$ expansion ratio $er\in\{3,4,6\}$ and kernel $k\in\{3,5\}$, train them from scratch for 200 epochs, and extract their final accuracy. Next, we compare three pretraining methods: Our pretraining involving 250 epochs of training the highest possible network, intitializing the super-network with these weights and fine-tuning it for 100 epochs using the multi-path sampling method, and two simple pretrainings of the network where the entire super-network is trained from scratch for 100 epochs, with and without multipath sampling method. We compare the accuracy of the extracted corresponding 18 networks from the different pretrained super-networks with the accuracy we got from training these networks from scratch, by computing the Kendal-Tau and Spearman metrics between them.  Since our method relay on the gradient of the loss with respect to the architectures parameters, it is important to have a pretraining that can rank the network correctly. In figure (\ref{fig:acc_kendal_tau}), we compare the accuracy of architecture extracted from our super-network with the robust pretraining and a simple pretraining against the accuracy of the same network trained from scratch. As we can see, using a more robust pretraining allows for the extracted architecture to have an accuracy (and hence a loss) that is much more correlated to the true accuracy of the extracted network. 
We compare the Kendall-Tau ($\tau$) and Spearman ($\rho$) correlations  between the accuracy of the networks extracted from the three pretrained super-networks (advanced and simple with and without multipath) and the accuracy of these networks from scratch. For a robust pretraining, the metric are $\tau=0.95, \rho=0.99$ while the latter for a simple multipath pretraining are $\tau=0.84, \rho=0.95$, and $\tau=0.35, \rho=0.44$ for a single-path simple pretraining. We can conclude that both our pretraining and sampling strategy allows to get a super-network whose accuracy of every extracted sub-network is strongly correlated to its accuracy from scratch. This observation justifies the fact that we do not update the weights of the super-network during the search.


% \subsection{Comparison with soft penalty}
% Todo: Add graphs where we see a jitter around the target latency when using TF-NAS penalty

\subsection{Outer Problem: Hard vs Soft Constraint}
\subsubsection{Toy Problem}
\label{subsec:toy_example}
In order to motivate the need for expressing the NAS problem using BCFW algorithm, we present a toy example based on quadratic programming. Our purpose is to solve the following optimization problem:
\begin{equation}
    \label{eqn:toy_ex}
    \begin{array}{l}
       \min_x \|x\|^2 \\
       \text{s.t}\\
       \sum_i x_i = 1
    \end{array}
\end{equation}
To this end, we can either use FW algorithm, or Gradient Descent (GD) with a hard penalty constraint, i.e. minimizing $\|x\|^2+\lambda \left(\sum_i x_i - 1\right)^2$ when $\lambda$ is a coefficient controlling the penalty. We use a dimensionality of $10$ for our problem, meaning that $x\in\mathbb{R}^{10}$. The solution of the problem can be computed analytically, and consists in a uniform vector whose all entries are $\frac{1}{d}$ where $d$, the dimension of the problem is 10 in our case, such as the optimal objective loss is $0.1$. In order to start with a feasible solution, we simply draw a random vector from uniform distribution and normalize its entries by dividing it by the sum of its components. One of the difficulties of using penalty loss is to tune the penalty coefficient $\gamma$, that represents the compromise between the minimization of the objective function and the respect of the constraint. In figure \ref{fig:fw_vs_gd}, we compare both objective and constraint losses for FW and GD with penalty algorithms. We can see that not only FW converges faster while respecting the constraint at every step of the optimization, it does not require to tune for an additional $\lambda$ parameter. When using GD with penalty, either the loss converges fast but not respecting the constraint (blue entries for $\lambda=1$) or the constraint is almost respected, but the convergences to the minimum is much slower than the FW one. In addition we can see that the constraint loss when using GD with hard penalty is never zero, even for higher values of $\lambda$.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{images/gd_diff_lambda.pdf}
    \caption{Objective loss and constraint loss of FW and hard penalty constraint GD for different values of hard penalty constraint $\lambda$. Continuous entries represent the objective loss (left y-axis) while dashed entries represent the constraint loss (right y-axis)}
    \label{fig:fw_vs_gd}
\end{figure}
\subsubsection{Ablation Study}

\subsection{Dataset and setting}
We apply our search method on the ImageNet Dataset, selecting $20\%$ of the training set as validation set. Our target device is a Intel XEON CPU, and we search for architectures with latencies $40, 45, 50, 55$ and $60$ milliseconds. For all of our experiments, we train our networks with SGD using label smoothing 0.1; mixup 0.2; Autoaugment; learning rate $0.1$; weight decay $10^{-4}$; and Nesterov momentum of $0.9$. We perform pretraining or our elastic network by first training the highest network (depth 4, expansion ratio 6, kernel 5) for 250 epochs and then fine-tuning the entire elastic network with 100 epochs. Unlike OFA that requires $250+3\times 120$ epochs, our procedure of pretraining requires only 350 epochs, since it is the ranking between the different sub-networks that matters rather than their final accuracy.
After our elastic network is pretrained, we apply our search method on a validation set composed by $20\%$ of the training set, and the search time is few GPU hours, since it requires only 6 epochs on the validation set, that is the equivalent in term of computational cost of a single epoch on the all training set.
\subsection{Comparisons with Current SOTA}
We test our method on Intel XEON CPU. For every of the networks we are comparing to, we take its official Pytorch implementation and measure the latency using a single thread without optimization such as MKL-DNN, in the exact same condition as for our networks. For this reason, the latency we report may differ from the latency reported in other papers, that may use optimization engine such as MKL-DNN or OpenVino. In order to have a fair comparison with methods not using robust pretraining, after an architecture is found, we train it from scratch in order to reflect the potential of our found architecture rather that the advantage of using a robust pretraining. We present our results in table \ref{tab:exp_cpu} and figure \ref{fig:acc_nas}. We can see that the latency of every found network corresponds to its target, and that the accuracy of the corresponding networks trained from scratch surpasses every other cited methods. In addition, in the second part of the table \ref{tab:exp_cpu} we present results with a pretraining that has followed the OFA progressive shrinking scheme, and with a fine tuning of 25 epochs after the architecture is found. As can be seen in table \ref{tab:exp_cpu}, our found network for $40$ ms latency reaches $74.8\%$ accuracy on ImageNet, that is $0.4\%$ better than TF-NAS-CPU-A \cite{TF-NAS}, $0.7\%$ better than SP-NASNET \cite{SPNAS} with similar or higher latency, while our $50$ ms latency network reaches $76.0\%$ accuracy, that is $0.9\%$ better than FB-NET \cite{fbnet}, $0.8\%$ better than MobileNetV3 \cite{mobilenetv3} and $0.3\%$ better than OFA \cite{OFA} with similar or higher latency. Our $55$ ms network reaches $76.9\%$ accuracy, that is $1.7\%$ higher that MNASNET-A1 \cite{tan2019mnasnet} whose search requires more than 90.000 GPU hours. Finally, our $60$ latency networks reaches $77.1\%$ accuracy, that is $1.3\%$ better than TF-NAS-CPU-B with similar latency, $0.6\%$ accuracy higher than MobileNet V2 \cite{mobilenetv2}, while being $10$ ms faster,  and just $0.2\%$ worse than EfficientNet B0 \cite{effnet} while being $25$ ms faster. 
In addition, in table \ref{tab:exp_GPU}, we also compare out method with others on NVIDIA P100 GPU.
\begin{table}[t]
    \centering
    \begin{tabular}{|l|c|c|}
    \hline 
    Model & latency (ms) & accuracy (\%) \\ \hline
         MobileNet v3 & 45 & 75.2 \\ \hline
         EfficientNet B0& 85 & 77.3 \\ \hline 
         TF-NAS-CPU A & 40 & 74.4 \\ \hline
         TF-NAS-CPU B & 60 & 75.8 \\ \hline
        %  MNAS-NET & 36 & 74.5 \\ \hline
         MNAS-NET A1 & 55 & 75.2 \\ \hline
         MNAS-NET B1 & 39 & 74.5 \\ \hline
         FB-NET & 47 & 75.1 \\ \hline
         SP-NASNET & 41 & 74.1 \\ \hline
         MobileNet v2 (x140) & 70 & 76.5 \\ \hline
         OFA & 42 & 75.7 \\ \hline
         \hline
         \multicolumn{3}{|l|}{Training from scratch} \\ \hline
         \textbf{Ours 40 ms} & 40 & 75.8 \\ \hline
         \textbf{Ours 45 ms} & 44 & 76.3 \\ \hline
         \textbf{Ours 50 ms} & 50 & 76.8 \\ \hline
         \textbf{Ours 55 ms} & 55 & 76.9 \\ \hline
         \textbf{Ours 60 ms} & 61 & 77.1\\ \hline
         \multicolumn{3}{|l|}{OFA pretraining, 25 epochs fine-tune} \\ \hline
         \textbf{Ours 40 ms} & 39 & 75.7 \\ \hline
         \textbf{Ours 45 ms} & 45 & 76.7 \\ \hline
         \textbf{Ours 50 ms} & 49 & 77.2 \\ \hline
         \textbf{Ours 55 ms} & 56 & 77.9 \\ \hline
         \textbf{Ours 60 ms} & 60 & 78.3 \\ \hline
         \hline
    \end{tabular}
    \caption{Imagenet Accuracy vs Latency on Intel Xeon CPU for a batch size of 1}
    \label{tab:exp_cpu}
\end{table}


\begin{table}[t]
    \centering
    \begin{tabular}{|l|c|c|}
    \hline 
    Model & latency (ms) & accuracy (\%) \\ \hline
         MobileNet v3 & 28 & 75.2 \\ \hline
         TF-NAS-GPU D & 30 & 74.2 \\ \hline
         \textbf{Ours 25 ms} & \textbf{27} & \textbf{75.7} \\ \hline \hline
         MNAS-NET B1 & 34 & 74.5 \\ \hline
         SP-NASNET & 36 & 74.1 \\ \hline
         TF-NAS-GPU B & 44 & 76.3 \\ \hline
         TF-NAS-GPU C & 37 & 75.2 \\ \hline
         MNAS-NET A1 & 37 & 75.2 \\ \hline
         FB-NET & 41 & 75.1 \\ \hline
         \textbf{Ours 30 ms} & \textbf{32} & \textbf{76.5} \\ \hline \hline
         TF-NAS-GPU A & 54 & 76.9 \\ \hline
         EfficientNet B0& 48 & \textbf{77.3} \\ \hline 
         MobileNet v2 (x140) & 50 & 76.5 \\ \hline
         \textbf{Ours 40 ms} & \textbf{41} & 77.1 \\ \hline
    \end{tabular}
    \caption{Imagenet Accuracy vs Latency on NVIDIA P100 GPU for a batch size of 64}
    \label{tab:exp_GPU}
\end{table}



\subsection{Effect of the projection}\label{sec:projection_effect}
As described in section \ref{sec:method}, after our method has converged, the continuous encoding of the accuracy might not belong to the original search space. If most methods simply take the arg-max of every encoding vector, this might lead to a sub optimal solution, either with lower or higher latency that required. In table \ref{tbl:projection}, we show the effect of our projection on the latency of the found network. As we can see, using our projection allows us to reach for a network much closer to the desired latency with less than $1$ ms difference with the required latency. This difference is mostly due to the fact that the search space is discrete and there is not always an architecture for every latency.

\begin{table}[t]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
    Expected & argmax & Projection
    \\
    \hline
    35 ms & 36 ms & 35 ms \\
    \hline
    40 ms & 42 ms & 40 ms \\
    \hline
    45 ms & 50 ms & 45 ms \\
    \hline
    50 ms & 54 ms & 49 ms \\
    \hline
    55 ms & 58 ms & 54 ms \\
    \hline
    60 ms & 66 ms & 60 ms \\
    \hline
    \end{tabular}
    \caption{Expected and real latency}
    \label{tbl:projection}
\end{table}

==> full_big_table.tex <==
\begin{table}[htb]
\small
    \centering
    \begin{tabular}{|l|c|c|c|c|}
    \hline
    Model & \makecell[c]{Size \\ ($10^6$)} & \makecell[c]{FLOPS \\ ($10^8$)} & \makecell[c]{Latency\\ (ms)} & \makecell[c]{Top-1 \\ (\%)}
    \\ \toprule
        %  \multirow{14}{*}{\rotatebox[origin=c]{90}{NVIDIA P100 GPU (batch:64)}}
        %  & MobileNetV3 & ?? & 2.2 & 28 & 75.2 \\ 
        %  & TFNAS-D & ?? & ?? & 30 & 74.2 \\ 
        %  & \textbf{Ours 25 ms} & ?? & ?? & \textbf{27} & \textbf{75.7}\\ \cline{2-6}
         
        %  & MnasNetA1 & ?? & 3.1 & 37 & 75.2 \\
        %  & MnasNetB1 & ?? & 3.1 & 34 & 74.5 \\ 
        %  & FBNet & ?? & 3.8 & 41 & 75.7 \\ 
        %  & SPNASNet & ?? & 3.3 & 36 & 74.8\\ 
        %  & TFNAS-B & ?? & ?? & 44 & 76.3 \\ 
        %  & TFNAS-C & ?? & ?? & 37 & 75.2 \\ 
        %  & \textbf{Ours 30 ms} & ?? & ??  & \textbf{32} & \textbf{77.3} \\ \cline{2-6} 
         
        %  & TFNAS-A & ?? & 3.0 & 54 & 76.9 \\ 
        %  & EfficientNetB0 & ?? & ??  & 48 & 77.3 \\ 
        %  & MobileNetV2 & ?? & ??  & 50 & 76.5 \\ 
        %  & \textbf{Ours 40 ms} & ?? & ??  & \textbf{41} & \textbf{77.9} \\ \midrule
         
        %  \multirow{15}{*}{\rotatebox[origin=c]{90}{Intel Xeon CPU (batch:1)}}
         
          MnasNetB1 & 4.4 & 3.1 & 39 & 74.5\\ 
          TFNAS-B & 4.9 & 2.3 & 40 & 75.0 \\ 
          SPNASNet & 4.4 & 3.3 & 41 & 74.9\\ 
          OFA CPU\footnotemark & 4.9 & 3.6  & 42 & 75.7 \\ 
          \textbf{Ours 40 ms} & 5.3 & 2.5 & 40 & 75.8\\ \cline{1-5}
         
         MobileNetV3 & 5.4 & 2.2 & 45 & 75.2 \\ 
         FBNet & 5.5 & 3.8 & 47 & 75.7 \\ 
         MnasNetA1 & 3.9 & 3.1 & 55 & 75.2 \\ 
         
         \textbf{Ours 45 ms} & 5.2 & 2.7 & 44 & 76.4\\ \cline{1-5}
         
         MobileNetV2 & 6.1 & 5.8 & 70 & 76.5 \\ 
         TFNAS-A & 7.1 & 3.0  & 60 & 76.5 \\ 
         \textbf{Ours 50 ms} & 7.5 & 2.9 & 50 & 77.1 \\ \cline{1-5}
         EfficientNetB0 & 5.3 & 3.9 & 85 & 77.3  \\ 
         \textbf{Ours 55 ms} & 8.1 & 3.3 & 55 & 77.6\\ \cline{1-5}
         FairNAS-C & 4.4 & 3.2 & 60 & 77.0 \\ 
         \textbf{Ours 60 ms} & 8.2 & 3.4 & 61 & 78.0\\ \hline
    \end{tabular}
    \caption{ImageNet top-1 accuracy, model size (number of parameters), FLOPS and latency comparison with other methods. The latency is reported for Intel Xeon CPU with a batch size of 1.}
    \label{tab:full_exp}
\end{table}\footnotetext{\label{fn:ofa}Finetuning a model obtained by 1200 GPU hours.}

% \addplot[color=red, mark=triangle*,very thick]coordinates {(2.2, 75.3)(2.5,75.8)(2.7, 76.4)(2.9, 77.1)(3.3, 77.6)(3.4,78.0)};\addlegendentry{Ours from scratch}

==> intro_v0.1.tex <==
\section{Introduction}
With the rise in popularity of Convolutional Neural Networks (CNN), the need for neural networks with fast inference speed and high accuracy, has been growing continuously. At first, manually designed architectures, such as VGG~\cite{VGG} or ResNet~\cite{ResNet}, targeted powerful GPUs as those were the common computing platform for deep CNNs. Many variants of those architectures were the golden standard until the need for deployment on edge devices or standard CPUs emerged. These are more limited computing platforms, calling for the design of lighter architectures. Furthermore, in practical scenarios there are often hard requirements on the real time latency or power consumption. This has spawned a new line of research aimed at finding architectures with both high performance and bounded resource demand. 

In order to deal with real time latency or power consumption constraints of edge devices or CPUs, Neural Architecture Search (NAS) has been aiming for the automatic design of lighter, and yet, highly accurate neural networks. Starting from unconstrained NAS, \cite{zoph2016neural, liu2018darts, cai2018proxylessnas}, a research branch of NAS has evolved, focusing on meeting a target latency over different platforms, e.g. TPU, CPU, Edge-GPU, FPGA, etc. While some methods heuristically formulate additional objectives to the loss for roughly controlling the latency \cite{tan2019mnasnet,fbnet, effnet, mobilenetv3}, or other indirect proxies such as FLOPS/MACS \cite{SNAS}, more recent methods aim for a strict satisfaction of latency constraints \cite{OFA, TF-NAS}. Latency constrained NAS aims at searching for the most accurate architecture that fully satisfies constraints over its inference time. 
The underlying constraints have to do with (1) the architecture admitting certain structural rules and (2) the resulted latency being lower than some upper bound.

Previous latency constrained NAS methods can be grouped into two categories: Reward based methods such as Reinforcement-Learning (RL) or Evolutionary Algorithm (EA) \cite{OFA,tan2019mnasnet, effnet, mobilenetv3}, where the search is performed by sampling several networks evaluated over some partial validation set to estimate the accuracy and latency forming a reward function. Latency-aware gradient based methods \cite{TF-NAS,fbnet} formulate a differentiable loss function consisting of an accuracy term and a proxy latency penalty term, thus the architecture can be directly optimized using the stochastic gradient descent (SGD) algorithm \cite{SGD} under the resulted trade-off. While the former relay heavily on accuracy and latency predictors that are expensive to acquire and oftentimes inaccurate, the latter incorporate a hard to tune trade-off between accuracy and latency that deteriorates the resulted accuracy without the latency requirement being fully met. This latency constraint is further violated due to the final discretization step projecting the resulted architecture from the differentiable search space to the discrete space of architectures.
 
In this paper, we propose a search algorithm that produces more accurate architectures for a strictly satisfied latency requirement (figure \ref{fig:acc_nas}), while maintaining a scalable search time to many platforms. The proposed algorithm is based on several key ideas, with the goal of formulating the problem more accurately, making less harmful assumptions, and fewer heuristics. 

 This is achieved by constructing a search space capable of parameterizing neural architectures with different operations, widths and depths in a fully differentiable manner. This space induces a one-shot model that is easy to train due to our novel multipath sampling over batch technique, such that every extracted sub-network is properly pretrained. We further suggest an accurate formula for the expected latency of every architecture residing in that space. Thus following a single straight forward pretraining of the one-shot model, we freeze the model's weights and search the space by iteratively solving a constrained optimization problem using the block coordinate stochastic Frank-Wolfe (BC-SFW) algorithm \cite{SFW,BCFW} while tightly satisfying the latency constraint anytime along the search, including the final discretization step, yet converges faster than SGD.
 
 Since the search is over a relatively small number of parameters, governing only the structure of the architecture, the efficient single pretrainig for all target platforms, followed by a fast search for every platform and latency requirement make our solution also scalable for many target devices and latency demands. 
 We believe that our formulation of NAS as a constrained optimization problem, equipped with efficient algorithms to be solved, will give raise to following work incorporating a variety of resource and structural constraints over the search space. 

==> introduction_pre.tex <==
\section{Introduction}
With the rise in popularity of Convolutional Neural Networks (CNN), the need for neural networks with fast inference speed and high accuracy, has been growing continuously. At first, manually designed architectures, such as VGG~\cite{VGG} or ResNet~\cite{ResNet}, targeted powerful GPUs as those were the common computing platform for deep CNNs. Variants of those architectures became the golden standard until the need for deployment on edge devices and standard CPUs emerged. These are more limited computing platforms, requiring lighter architectures that for practical scenarios must comply with hard constraints on real time latency or power consumption. This has spawned a line of research aimed at finding architectures with both high performance and bounded resource demand. 

The main approaches to solve this evolved from Neural Architecture Search (NAS)~\cite{zoph2016neural, liu2018darts, cai2018proxylessnas}, while adding a constraint on the target latency over various platforms, e.g., TPU, CPU, Edge-GPU, FPGA, etc. 
The constrained-NAS methods can be grouped into two categories: (i) Reward based methods such as Reinforcement-Learning (RL) or Evolutionary Algorithm (EA) \cite{OFA,tan2019mnasnet, effnet, mobilenetv3}, where the search is performed by sampling networks and predicting their final accuracy and resource demands by evaluation over some validation set. The predictors are made of complicated models and hence require many samples and sophisticated fitting techniques~\cite{white2021powerful}. Overall this makes those oftentimes inaccurate, expensive to acquire, and hard to optimize as objective functions due to their complexity. (ii) Resource-aware gradient based methods formulate a differentiable loss function consisting of a trade-off between an accuracy term and either a proxy soft penalty term~\cite{TF-NAS,fbnet} or a hard constraint~\cite{nayman2021hardcore}. Therefore, the architecture can be directly optimized via bi-level optimization using stochastic gradient descent (SGD)~\cite{SGD} or stochastic Frank-Wolfe (SFW)~\cite{hazan2016variance}. However, the bi-level nature of the problem introduces many challenges~\cite{P-DARTS,DARTS+,noy2020asap, nayman2019xnas} and recently~\cite{wang2021rethinking} pointed out the inconsistencies associated with using gradient information as a proxy for the quality of the architectures, especially in the presence of skip connections in the search space.

In this paper, we propose a search algorithm that produces architectures with high accuracy that strictly satisfy any given hard latency constraint.
 The search algorithm is fast and scalable to a large number of platforms and does not rely on gradients as a proxy for the quality of the architectures. 
 
The proposed algorithm is based on two key ideas, with the goal of formulating a simple quadratic optimization objective which is interpretable, easier to optimize and relying less on gradient information:

 (1) We propose a simple and well preforming quadratic accuracy estimator which is interpretable, easy to optimize and cheap to acquire by sampling as many selected sub-networks from a one-shot model~\cite{bender2018understanding, fairnas, SPOS, OFA, nayman2021hardcore} as the number of decision variables. Many insights about the contribution of different design choices can be extracted due to the way it is constructed. We additionally propose an alternative learnable version of such a predictor, which performs even better and is as easy to optimize, however, it lacks interpretability and is more expensive to compute. 
 \\(2) The quadratic form of both predictors allows the formulation of the latency constrained NAS problem as an \textit{Integer Quadratic Constrained Quadratic Programming} (IQCQP) and thus we utilize two off-the-shelf algorithms and a designated one to efficiently solve it.
 
 The optimization approach we propose has several advantages. First, the outcome networks provide high accuracy and closely comply to the latency constraint. 
 In addition, our solution is scalable to multiple target devices and latency demands. This scalability is due to the formulation of the problem as a QCQP and the application of dedicated algorithms to solve it within several minutes over a common CPU.

==> multipath_code.tex <==
\begin{figure}[htb]
\begin{lstlisting}[language=Python]
import torch
from torch.nn.functional import gumbel_softmax

def multipath(a, ops, x):
    assert C = len(a) == len(ops)
    bs = x.shape[0]
    a = torch.log(a).repeat(bs)
    a = a.reshape(bs, C).transpose(0, 1)
    a_hat = gumbel_softmax(a)

    o = torch.zeros_like(x)
    for ah, op in in zip(a_hat, ops):
        o += ah.view(-1, 1, 1, 1) * op(x)
    
    return o
\end{lstlisting}
\caption{PyTorch Multipath Code}\label{code:multipath}
\end{figure}


    % logits = torch.log(a).repeat(batch_size).reshape(batch_size, C).transpose(0, 1)

==> prel_cvpr.tex <==
\makeatletter
\@namedef{ver@everyshi.sty}{}
\makeatother

% \usepackage{float}
% \usepackage{wrapfig}
% \usepackage{subfig}
%\usepackage{cite}
% \usepackage[ansinew]{inputenc}
% \usepackage[T1]{fontenc}
\usepackage[dvipsnames,table,xcdraw]{xcolor}
% \usepackage{microtype}
\usepackage{graphicx}
\usepackage{graphics}
%\DeclareGraphicsExtensions{.jpg,.eps,.gif}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{bm}
\usepackage{pgfplots}
\usepackage{adjustbox}
\usepackage{enumerate}
\usepackage{textcomp}
\usepackage{tikz}
\usepackage{tabu}
\usepackage{caption}
%\captionsetup{labelsep=period}
\usetikzlibrary{shapes, arrows, decorations.text, shadows.blur, backgrounds, positioning,fit,calc}
% \usepackage{float}
% \restylefloat{table}
% \usepackage{lmodern}



\usepackage{array} % and/or
\usepackage{longtable} % and/or
% \usepackage{colortab} % or
% \usepackage{colortbl}
% \usepackage{arydshln}
\pgfplotsset{compat=1.16}
\usepackage{microtype}
% \usepackage{textcomp}
\usepackage{multirow}
\usepackage{makecell} 
%\usepackage{subcaption} 
\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\usepackage{booktabs} % for professional tables
% \usepackage[english]{babel}
\usepackage{algorithmic}
\usepackage{algorithm}
\usepackage{amsmath,amssymb,amsthm}
\usepackage{mathtools}

\newtheorem{de}{Definition}[section]
\newtheorem{theo}{Theorem}[section]
\newtheorem{prop}{Proposition}[section]
\newtheorem{lem}[theo]{Lemma}
\newenvironment{remark}[1][Remark]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
\newcommand{\argmax}{\operatornamewithlimits{argmax~}}
\newcommand{\argmin}{\operatornamewithlimits{argmin~}}
\newcommand{\sinc}{\operatorname{sinc}}
\newcommand{\comb}{\operatorname{comb}}
\newcommand{\prox}[2]{\operatorname{\mathbf{prox}}_{#2}\left(#1\right)}
\newcommand{\rect}{\operatorname{rect}}
\newcommand{\erf}{\operatorname{erf}}
\newcommand{\diver}{\operatorname{div}}
\newcommand{\sgn}{\operatorname{sign}}
\newcommand{\dom}{\operatorname{dom}}
\newcommand{\trace}{\operatorname{trace}}
\newcommand{\interior}{\operatorname{int}}
\newcommand{\off}{\operatorname{off}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\mean}{\operatorname{mean}}
%\newcommand{\L}{\mathbf{L}}
\newcommand{\B}{\mathbf{B}}
\newcommand{\M}{\mathbf{M}}
\newcommand{\F}{\mathbf{F}}
\newcommand{\HH}{\mathbf{HH}}
\newcommand{\W}{\mathbf{W}}
\newcommand{\D}{\mathbf{D}}
\newcommand{\X}{\mathbf{X}}
\newcommand{\s}{\mathbf{S}}
\newcommand{\p}{\mathbf{P}}
\newcommand{\pp}{\mathbf{p}}
\newcommand{\uu}{\mathbf{u}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\xx}{\mathbf{x}}
\newcommand{\Q}{\mathbf{Q}}
\newcommand{\U}{\mathbf{U}}
\newcommand{\V}{\mathbf{V}}
\newcommand{\J}{\mathbf{J}}
\newcommand{\I}{\mathbf{I}}
\newcommand{\LL}{\mathbf{L}}
\newcommand{\PHI}{\bm{\Phi}}
\newcommand{\PSI}{\mathbf{\Psi}}
\newcommand{\LAMBDA}{\bm{\Lambda}}
\newcommand{\GAMMA}{\bm{\Gamma}}
\newcommand{\Alpha}{\bm{\alpha}}
\newcommand{\Beta}{\bm{\beta}}
\newcommand{\A}{\mathbf{A}}
\newcommand{\mb}[1]{{\boldsymbol{#1}}}
\newcommand{\vw}{\mb{w}}
\newcommand{\vb}{\mb{b}}
\newcommand{\vu}{\mb{u}}
\newcommand{\ve}{\mb{e}}
\newcommand{\vy}{\mb{y}}
\usepackage{bbm}
% \newcommand{\aalpha}{\boldsymbol{\alpha}}
\newcommand{\balpha}{\bm{\alpha}}
\newcommand{\bbeta}{\bm{\beta}}
\newcommand{\btau}{\bm{\tau}}
\newcommand{\brho}{\bm{\rho}}

\newcommand{\bgamma}{\bm{\gamma}}
\newcommand{\bdelta}{\bm{\delta}}
\newcommand{\bDelta}{\bm{\Delta}}
\newcommand{\bs}{\bm{s}}

\newenvironment{disarray}%
 {\everymath{\displaystyle\everymath{}}\array}%
 {\endarray}
% \everymath{\displaystyle\everymath{}}
\usepackage{pgfpages}



\newcommand{\norm}[1]{\lVert #1 \rVert}
%\newcommand{\angle}{\operatorname{angle}}
\usepackage{relsize}
\usepackage{lmodern}


\setlength{\intextsep}{0em}
\setlength{\parskip}{0.3em}
\setlength{\dblfloatsep}{-3em}
\setlength{\dbltextfloatsep}{-3em}

\setlength{\abovecaptionskip}{0.7em}
\setlength{\belowcaptionskip}{-1em}
\usepackage[nodisplayskipstretch]{setspace}
\setstretch{0.95}

\AtBeginDocument{%
  \setlength\abovedisplayskip{3pt}
  \setlength\belowdisplayskip{3pt}
  }



\usepackage{listings}

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}

\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},   
    commentstyle=\color{codegreen},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\ttfamily\footnotesize,
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    keepspaces=true,                 
    numbers=left,                    
    numbersep=5pt,                  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=2
}

\lstset{style=mystyle}
\definecolor{darkbluetemp}{rgb}{0,0.08,0.45}
% \usepackage[colorlinks=true, allcolors=darkbluetemp]{hyperref}

